POD: A Smartphone That Flies

We present POD, a smartphone that flies, as a new way to achieve hands-free, eyes-up mobile computing. Unlike existing drone-carried user interfaces, POD features a smartphone-sized display and the computing and sensing power of a modern smartphone. We share our experience in building a prototype of POD, discuss the technical challenges facing it, and describe early results toward addressing them.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
